Graph Spectral Image Processing

Recent advent of graph signal processing (GSP) has spurred intensive studies of signals that live naturally on irregular data kernels described by graphs (e.g., social networks, wireless sensor networks). Though a digital image contains pixels that reside on a regularly sampled 2D grid, if one can design an appropriate underlying graph connecting pixels with weights that reflect the image structure, then one can interpret the image (or image patch) as a signal on a graph, and apply GSP tools for processing and analysis of the signal in graph spectral domain. In this article, we overview recent graph spectral techniques in GSP specifically for image / video processing. The topics covered include image compression, image restoration, image filtering and image segmentation.

==> filter.tex <==
As in image denoising and other inverse imaging, extracting smooth components of the image, i.e., low-graph-frequency components, is a critical issue since many image filtering applications utilize edge-preserving image smoothing as a key ingredient. First, we describe some early works on graph spectral smoothing of images/3-D objects, and then recent edge-preserving smoothing methods are presented. As applications, non-photorealistic rendering of images is introduced. Fast computation methods are also described.

\subsection{Smoothing and Diffusion in Graph Spectral Domain}
%In the graph spectral analysis for image processing, it basically decomposes image components based on the spectrum of the image structure, e.g., graph Laplacian. 

One of the seminal works on smoothing using graph spectral analysis is 3-D mesh processing from computer graphics community \cite{taubin95, taubin96}\footnote{The term ``graph signal" was first introduced in \cite{taubin96}, to the best of our knowledge.}. It determines edge weights of the graph as Euclidean distance between vertices (of the 3-D mesh) and smooths the 3-D mesh shape using a graph low-pass filter with a binary response. That is, the spectral response of the filter is
\begin{equation}
\label{eqn:taubinfilter}
\widetilde{h}(\lambda_k) = \begin{cases}
1      & \text{if } k \le T_k, \\
0      & \text{otherwise},
\end{cases}
\end{equation}
where $T_k$ is the user-defined bandwidth, i.e., how many eigenvalues are passed. Clearly, we can define an arbitrary response according to the purpose. This kind of naive approaches have been used in several computer graphics/vision tasks \cite{zhang10, vallet08, desbrun99, fleishman03, kim05}. The filter in \eqref{eqn:taubinfilter} actually smoothes out high-graph-frequency components, however, as the number of vertices grows, it is difficult to compute graph Fourier basis via eigendecomposition.
% Spectral approaches for geometry processing of the 3-D meshes like deformation have been presented in \cite{vallet08, desbrun99, fleishman03, kim05}.

Heat kernel in the spectral domain has also been proposed in \cite{zhang08}. In this work, the weight of the edges of the graph is computed according to photometric distance, i.e., large weights are assigned to the edges whose both ends have similar pixel values and vice versa. Additionally, its graph spectral filter is defined as a solution of the heat equation on the graph as follows:
\begin{equation}
\label{eqn:heatkernel}
\widetilde{h}(\lambda) = e^{-t\lambda},
\end{equation}
where $t > 0$ is an arbitrary parameter to control the spreading speed due to diffusion. By implementing it with the naive approach, it still needs a large computation cost due to eigendecomposition of graph Laplacian. However, \eqref{eqn:heatkernel} can also be represented by using Taylor series around the origin as
\begin{equation}
\label{eqn:heat_taylor}
e^{-t\lambda} = \sum_{k=0}^{\infty} \frac{t^k}{k!} (-\lambda)^k.
\end{equation}
By truncating the above equation with an arbitrary order, we can approximate it as a finite-order polynomial \cite{hammond11, shuman13}. In \cite{zhang08}, the Krylov subspace method is used along with \eqref{eqn:heat_taylor} to approximate the graph filter.

However, as shown in Fig. \ref{fig:approxerror}, its approximation accuracy significantly gets worse for large $\lambda$. Since the maximum eigenvalue $\lambda_{\max}$ highly depends on the graph used, it is better to use different approximation methods (introduced in Section \ref{subsec:fastcomp}).

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig_yt/taylor_vs_chebyshev.eps}
\caption{Approximation error comparison of $\widetilde{h}(\lambda) = e^{-\lambda}$.}
\label{fig:approxerror}
\end{figure}

\subsection{Edge-Preserving Smoothing}
As previously mentioned, edge-preserving smoothing is widely used for various image filtering tasks as well as image restoration \cite{nagao79, pomalaza-raez84, weickert98, tomasi98, barash02, durand02, farbman08, xu11, he13}. Image restoration aims to get the ground-truth image (approximately) from its degraded version, whereas edge-preserving smoothing is used to yield a user-desired image from the original one; It is either noisy or noise-free.

In the graph setting, we need to define pixel-wise or patch-wise relationships as a distance between pixels or patches, and it is used to construct a graph. Three distances are considered in general \cite{milanfar13}: 1) geometric distance, 2) photometric distance, and 3) these combination.
% Since the structure of the image has to be preserved as accurate as possible after smoothing, the graph must be constructed by taking into consideration of photometric distance. 
Furthermore, especially for image filtering other than restoration, we often employ 4) \textit{saliency} of the image/region/pixel, which simulates perceptual behavior \cite{itti98, harel06}.

The graph spectral representation of bilateral filter \cite{gadde13} introduces that the bilateral filter can be regarded as a combination of  graph Fourier basis and a graph low-pass filter. The filter coefficients of the bilateral filter is represented in \eqref{eq:edgeWeight}.
%Let $\mathbf{t}_i \in \mathbb{R}^2$ be the coordinate of $x_i$. It is well known that the bilateral filter \cite{tomasi98} computes its output as
%\begin{equation}
%\label{eqn:graphbf}
%\widehat{x}_i = \frac{1}{d_i}\sum_{j} w_{ij} x_j
%\end{equation}
%where
%\begin{equation}
%\label{ }
%w_{ij}= \exp\left(-\frac{||\mathbf{t}_i - \mathbf{t}_j||^2_2}{2\sigma_d^2}\right)\exp\left(-\frac{(x_i - x_j)^2}{2\sigma_r^2}\right),
%\end{equation}
%and $d_i = \sum_j w_{ij}$ is a scaling term. We can control the smoothing strength of the bilateral filter by changing the parameters $\sigma_d$ and $\sigma_r$. 
Since its weights clearly depend on the geometric and photometric distances, it is a pixel-dependent filter. 

In a classical sense, the frequency domain representation of the bilateral filter cannot be calculated straightforwardly. In contrast, the bilateral filter can be considered as a graph filter by considering a weight matrix $\mathbf{W}$ where $[\mathbf{W}]_{ij} = w_{i,j}$ as an adjacency matrix of the graph. \eqref{eq:edgeWeight} is rewritten as
\begin{equation}
\label{ }
\widehat{\mathbf{x}} = \mathbf{D}^{-1}\mathbf{W} \mathbf{x}
\end{equation}
where $\mathbf{D} = \text{diag}(d_0, d_1, \ldots, d_{N-1})$ in which $d_i = \sum_j w_{i,j}$. It is further rewritten as a graph spectral filter by
\begin{equation}
\label{ }
\widehat{\mathbf{x}} = \mathbf{D}^{-1/2}\mathbf{U}_n(\mathbf{I} -\mathbf{\Lambda}_n)\mathbf{U}^T_n\mathbf{D}^{1/2}\mathbf{x}
\end{equation}
%
%\begin{equation}
%\label{ }
%\begin{split}
%\widehat{\mathbf{x}} &= \mathbf{D}^{-1}(\mathbf{D} -\mathbf{L}) \mathbf{x}\\
%& = \mathbf{D}^{-1}\mathbf{D}^{1/2}(\mathbf{D} -\mathbf{D}^{-1/2}\mathbf{L}_n\mathbf{D}^{-1/2}) \mathbf{D}^{1/2}\mathbf{x}\\
%& = \mathbf{D}^{-1/2}\mathbf{U}_n(\mathbf{I} -\mathbf{\Lambda}_n)\mathbf{U}^T_n\mathbf{D}^{1/2}\mathbf{x},
%\end{split}
%\end{equation}
where we utilize the fact $\mathbf{W} = \mathbf{D} -\mathbf{L}$ and $\mathbf{L}_n = \mathbf{D}^{-1/2}\mathbf{L}\mathbf{D}^{-1/2}$. When we define a degree-normalized signal as $\underline{\mathbf{x}} = \mathbf{D}^{-1/2}\mathbf{x}$, the above equation is represented as
\begin{equation}
\label{ }
\underline{\widehat{\mathbf{x}}} = \mathbf{U}_n\widetilde{h}_\text{BF}(\mathbf{\Lambda}_n)\mathbf{U}^T_n\underline{\mathbf{x}},
\end{equation}
where $\widetilde{h}_\text{BF}(\lambda_n) = 1 - \lambda_n$. Since $\lambda_n \in [0, 2]$, it acts as a graph low-pass filter.

The above-mentioned representation of the bilateral filter suggests that the original bilateral filter implicitly designs the graph Fourier basis and the graph spectral filter simultaneously. For example, consider the following spectral response:
\begin{equation}
\label{eqn:graphfilter_denoising}
\widetilde{h}(\lambda) = \frac{1}{1 + \rho \widetilde{h}_r(\lambda)},
\end{equation}
where $\widetilde{h}_r(\lambda)$ is a graph high-pass filter and $\rho > 0$ is a parameter. Clearly $\widetilde{h}(\lambda)$ works as a graph low-pass filter. It is the optimal solution of the following denoising problem \cite{gadde13}:
\begin{equation}
\label{ }
\argmin_{\underline{\mathbf{x}}} ||\underline{\mathbf{y}} - \underline{\mathbf{x}}||_2^2 + \rho||\mathbf{H}_r  \underline{\mathbf{x}}||_2^2,
\end{equation}
where $\mathbf{y} = \mathbf{x} + \mathbf{e}$ in which $\mathbf{e}$ is a zero-mean i.i.d. Gaussian noise and $\mathbf{H}_r = \mathbf{U} \widetilde{h}_r(\mathbf{\Lambda})\mathbf{U}^T$.

It is known that the bilateral filter sometimes needs many iterations to smooth out details for textured and/or noisy images. To boost up the smoothing effect, the trilateral filter method \cite{choudhury03} first smoothes gradients of the image, and then the smoothed gradient is utilized to smooth intensities. Its counterpart in the graph spectral domain has also proposed in \cite{onuki16} with the parameter optimization method for $\rho$ in \eqref{eqn:graphfilter_denoising} which minimizes MSE after denoising.

The power of graph spectral analysis for image filtering is that it is able to consider the prior information of the image, e.g., edges, textures, and saliencies, as a graph, separately from the user-desired information as a graph spectral response. That is, we can (and need to) design good graphs as well as graph filters for the desired image filtering effects.

The above approach is generally represented as
\begin{equation}
\label{eqn:psdfilter}
\widehat{\mathbf{x}} = \mathbf{W}\widetilde{h}(\mathbf{\Lambda})\mathbf{W}^{-1}\mathbf{x},
\end{equation}
where $\mathbf{W} \in \mathbb{R}^{N \times N}$ is an arbitrary dictionary which sparsely represents the image $\mathbf{x}$ \footnote{Generally the number of atoms in the dictionary could be overcomplete, but we focus on the square and invertible $\mathbf{W}$ for the sake of simplicity.} and $\widetilde{h}(\mathbf{\Lambda}) = \text{diag}(\widetilde{h}(\lambda_0), \widetilde{h}(\lambda_1), \ldots)$ is a filter in the spectral domain (not restricted to the spectrum of the graph). This general form is considered in a modern image processing tasks \cite{milanfar13} where $\mathbf{W}$ and $\mathbf{\Lambda}$ are obtained from a (symmetrized) matrix whose elements are come from arbitrary image processing. However, in this paper, we focus on a specific form of \eqref{eqn:psdfilter} in graph setting, where the dictionary is so-called graph Fourier basis and the spectral response is designed for the eigenvalues of the graph.

\begin{figure}[t]
\centering
\subfigure{\includegraphics[width=.53\linewidth]{fig_yt/flower_original.png}}\ \subfigure{\includegraphics[width=.45\linewidth]{fig_yt/mountain_original.png}}
\subfigure{\includegraphics[width=.53\linewidth]{fig_yt/flower_smoothed.png}}\ \subfigure{\includegraphics[width=.45\linewidth]{fig_yt/mountain_smoothed.png}} 
\subfigure{\includegraphics[width=.53\linewidth]{fig_yt/flower_stylized.png}}\ \subfigure{\includegraphics[width=.45\linewidth]{fig_yt/mountain_pencil.png}}
\caption{Examples of non-photorealistic rendering. Image stylization is shown in the left column and pencil drawing is shown in the right column. From top to bottom: Original, edge-preserving smoothing, and NPR results, respectively. The multiscale method in \cite{yagyu16} is used for edge-preserving smoothing. For stylization, luminance component of the smoothed image is quantized and the edge image is combined with it. For pencil drawing, edge detection is performed to the smoothed image and the edge image is combined with the high-frequency information in the image. Both test images are obtained from \protect\url{https://pixabay.com/}.}
\label{fig:npr_example}
\end{figure}

\subsection{Edge-Preserving Smoothing and Retargeting as Graph Signal Processing}
For various image processing tasks including the topics described in this paper, filtering methods combining geometric and photometric distances and saliency have been proposed (see \cite{tomasi98, buades05, buades05a, takeda07, bhat10, paris11, milanfar13, he13, aubry14} and references therein). Among the works, \textit{domain transform} \cite{gastal11, gastal15} has a unique approach: It transforms the photometric distance  into the geometric distance, then the nonuniformly distributed discrete signal is low-pass filtered. Finally, the nonuniformly distributed signal is warped to its original pixel position to obtain the resulting smoothed image.

Formally, the domain transform for a 1-D signal is performed in the following steps.
\begin{enumerate}
  \item Compute a warped pixel position according to the geometric and photometric distances.
\begin{equation}
\label{ }
t_i  = t_{i-1} + \alpha_g + \alpha_p \sum_{k=0}^{N_c - 1} |x^{(k)}_i - x^{(k)}_{i-1}|,
\end{equation}
where $t_i$ is the $i$th pixel position ($t_0 = 0$), $\alpha_g$ and $\alpha_p$ are the weights for the geometric and photometric distances (usually $\alpha_g = 1$), respectively, $x^{(k)}_i$ is the $i$th pixel value of the $k$th color component, and $N_c$ is the number of color channels, e.g., $N_c = 3$ for RGB color images.
  \item Place $x_i$ onto $t_i$ as $f(t_i) := x_i$. At this time, $f(t_i)$ can be regarded as a nonuniformly sampled continuous signal.
  \item Perform a low-pass filter $h(t)$ to $f(t_i)$ to obtain $\widehat{f}(t) = h(t) \ast f(t)$ defined in the continuous domain $t \in [0, t_{N-1}]$.
  \item Replace the filtered signal $\widehat{f}(t_i)$ back to its original coordinates, i.e., $\widehat{x}_i = \widehat{f}(t_i)$.  
\end{enumerate}
The motivation of the domain transform is clearly shared with that of the graph-based image processing; The relationship between signal values is determined first, then the low-pass filter is performed to obtain user-desired effects.

The deformed pixel position $t_i$ can also be regarded as a solution of the following linear problem \cite{yagyu16}.
\begin{equation}
\label{eqn:domaintransmatrix}
\mathbf{\Psi} \mathbf{t} = \bm{\tau},
\end{equation}
where
\begin{equation}
\label{}
[\mathbf{\Psi}]_{ij} = \begin{cases}
1      & i = j, \\
-1 &  i = j-1,\\
0     & \text{otherwise}
\end{cases}
\end{equation}
and $\tau_i = \alpha_g + \alpha_p \sum_{k=0}^{N_c - 1} |x^{(k)}_{i} - x^{(k)}_{i-1}|$. \eqref{eqn:domaintransmatrix} can be solved by simply taking the inverse of $\mathbf{\Psi}$ and it is represented as
\begin{equation}
\label{ }
\mathbf{\Psi}^{-1} = \begin{bmatrix}
1 & 0 & \cdots & \\
1 & 1 & \ddots & \\
\vdots & \ddots & \ddots \\
\end{bmatrix}.
\end{equation}

Here, let us consider the following optimization problem:
\begin{equation}
\label{}
\argmin_{\mathbf{t}}||\bm{\tau} - \mathbf{\Psi}\mathbf{t}||^2_2.
\end{equation}
Its solution is $\mathbf{\Psi}^T\mathbf{\Psi} \mathbf{t} = \mathbf{\Psi}^T\bm{\tau}$ and \eqref{eqn:domaintransmatrix} is obtained when we multiply $\mathbf{\Psi}^{-T}$ for both sides. Interestingly, the above linear problem can also be represented as
\begin{equation}
\label{eqn:Lpathx}
\mathbf{L}_{\text{path}} \mathbf{t} - \bm{\tau}' = \mathbf{0},
\end{equation}
where $\mathbf{L}_{\text{path}} = \mathbf{\Psi}^T\mathbf{\Psi}$ is the graph Laplacian of the path graph and $\tau'_i = \alpha_p \sum_{k=0}^{N_c - 1} |x^{(k)}_{i+1} - x^{(k)}_{i}| - |x^{(k)}_{i} - x^{(k)}_{i-1}|$. It means we can define a generalized version of the domain transform and the general form is very closely related to various mesh deformation methods \cite{gu02, desbrun02, zhang10, rong08, wang08}.

Mesh deformation is widely used in computer graphics and vision as well as image processing. The simplest form of the optimization problem can be formulated as follows \cite{sorkine04, zhou05, wang08}:
\begin{equation}
\label{eqn:meshdeform}
\mathbf{L}_1 \mathbf{p}' - \mathbf{L}_0 \mathbf{p} = \mathbf{0}
\end{equation}
where $\mathbf{L}_0$ and $\mathbf{L}_1$ are, respectively, the graph Laplacians for the original and deformed vertices of the mesh and $\mathbf{p}$ and $\mathbf{p}'$ are the original and deformed vertex coordinates, respectively. Since a pure Laplacian is a singular matrix, \eqref{eqn:meshdeform} needs constraints to obtain robust solutions. One of the widely-used constraints is the boundary condition which keeps the deformed vertex positions on the boundary unchanged.

\eqref{eqn:Lpathx} is a special version of \eqref{eqn:meshdeform} since $\mathbf{t}'$ in \eqref{eqn:Lpathx} represents the second-order differentiation of the deformed pixel position. Conversely, if we can define a ``good" distance (depending on applications) between a pair of pixels, its deformed pixel position would be determined by solving a linear equation having the form like \eqref{eqn:meshdeform}, as long as the overall cost function is quadratic. The desired pixel values could be obtained by a graph-based filtering.

If we perform a low-pass filter to the nonuniformly distributed pixel $f(\mathbf{t}'_i)$ then move it back to its original uniform-interval position, the graph-based filtering is an edge-preserving smoothing. Instead of that, if we interpolate the uniform-interval pixels $\widehat{f}(\mathbf{t}_i)$ from $f(\mathbf{t}'_i)$, it is so-called content-aware image resizing, also known as \textit{image retargeting} \cite{wolf07, wang08, zhang09shape}. Their relationship is illustrated in Fig. \ref{fig:smoothing_retargeting}.

Note that the conventional approaches need to consider signal processing in a continuous domain as a counterpart of the discrete domain where image signals exist. It leads to that we have to estimate the appropriate continuous domain from the input signal or any other prior information. Generally it is a difficult task and requires a large computation cost due to signal processing in the continuous domain. In contrast, graph-based methods are fully discretized; memory and computation costs are usually kept low. Additionally, the prior information is appropriately utilized to construct/learn a graph for purposes.

\begin{figure*}[t]
\centering
\includegraphics[width=.9\linewidth]{fig_yt/smoothing_retargeting.eps}
\caption{Relationship between edge-preserving smoothing and image retargeting as signal processing on nonuniform grid. Graph signal processing corresponds to the construction of the appropriate graph and filtering of the nonuniformly sampled signal.}
\label{fig:smoothing_retargeting}
\end{figure*}

% note that $\mathbf{\Psi}^T\mathbf{\Psi} = \mathbf{L}_{\text{path}}$


%and interestingly, it becomes
%\begin{equation}
%\label{ }
%\mathbf{\Psi}^T\mathbf{\Psi} \mathbf{x} = \mathbf{L}_{\text{path}} \mathbf{x} = \mathbf{t}.
%\end{equation}
%Therefore, $\mathbf{x}$ in this case can be obtained by a graph filter $\widetilde{h}(\lambda) = 1/\lambda$. As in the case of the bilateral filter and its variants, this spectral response can be changed according to the desired output. Note that this determines the deformed pixel position, not the pixel value itself. 
%
%This original domain transform is a uni-directional differentiation for the purpose being $x_0 = 0$ and its calculation faster. But more generally, bi-directional deformation can also be considered and it has a Laplacian form of $\mathbf{\Psi}$ as
%\begin{equation}
%\label{ }
%\mathbf{\Psi} = \begin{bmatrix}
%1 & -1 &  & & \\
%-1 & 2 & -1 &   &  \\
%  & & \ddots &  &\\
%& &-1& 2&-1\\
%  && & -1 & 1\\ 
%\end{bmatrix}.
%\end{equation}
%This is obviously the graph Laplacian of the path graph.

%The pixel domain deformation can be represented as the following linear equation \cite{}:
%\begin{equation}
%\label{ }
%\mathbf{x} = \mathbf{\Psi} \mathbf{t},
%\end{equation}
%where
%\begin{equation}
%\label{ }
%test.
%\end{equation}
%Since $\mathbf{\Psi}$ is a square lower triangular matrix with nonzero diagonal elements, it is always invertible. In other words, $\mathbf{x}$ is the solution of the following optimization problem.
%\begin{equation}
%\label{ }
%\argmin_{\mathbf{x}} ||\mathbf{\Psi}^{-1}\mathbf{x} - \mathbf{t}||^2_2.
%\end{equation}
%The original domain transform is a uni-directional deformation, i.e., $x_0 = 0$, since the edge-preserving smoothing is being faster. But more generally, bi-directional deformation can also be considered.

%\subsection{Other Applications}
%Other NPR applications includes stylization, which yields cartoon-like images whose separated regions have piecewise-smooth characteristics \cite{Gastal2011, Yagyu2016, Yagyu2016a, Sadrea2017}. Stylization can be obtained with the graph-based method mentioned above, whose edge weights between regions are very small and the passband of the lowpass filter is very narrow. Abstraction is similarly done by replacing the lowpass filter with a broader passband than that for stylization.

\subsection{Non-Photorealistic Rendering of Images}
Edge-preserving smoothing is also widely used in non-photorealistic rendering (NPR), which is one of key tasks in computer graphics. With a combination of image processing techniques like thresholding (both in spatial and frequency domains) and segmentation, NPR accomplishes various artificial effects such as stylization, pencil drawing, and abstraction \cite{winkenbach94, strothotte02, rusinkiewicz08, gastal11, yagyu16, yagyu16a, sadreazami17}. Examples of NPR are shown in Fig. \ref{fig:npr_example}.

Sometimes one needs NPR images with different degrees of artificiality. We can accomplish them by defining different graphs and filters for different artificialities, however, it is generally a cumbersome process. Instead, multiscale decomposition of images would be an alternative way. Traditionally, each scale represents an image component which has a specific frequency range. In contrast, graph-based multiresolution has more flexibility on the preserved component in each scale; It can also reflect the structure of pixels in each scale. For example, when we apply graph Laplacian pyramid \cite{shuman16} to an image with an appropriate multiscale graph and graph filters, high-graph-frequency component represents pixel-level fine details, while the upper (coarser) level component has region-level features. By changing functions to strengthen and weaken the transformed coefficients in each scale, we can obtain different NPR results from one multiscale representation of images. The multiscale representation has been proposed in the literature \cite{rong08, zhang10, yagyu16}.

\subsection{Fast Computation}
\label{subsec:fastcomp}
Fast computation of graph spectral filtering is a key for its practical applications since the modern image filtering, including graph spectral filters, treats image signals as one long-vector $\mathbf{x} \in \mathbb{R}^{WH}$ where $W$ and $H$ are the width and height of the original image, respectively. Image resolution of digital broadcasting is becoming larger and larger; For example, 4K ultra-high-definition corresponds to $W = 3840$ and $H = 2160$ pixels, which leads to $WH > 8 \times 10^{6}$. As the naive approach, we have to construct a graph Laplacian of the size $WH \times WH$, then perform its eigendecomposition. This approach needs huge computational burden even in recent high-spec computers, and therefore, a workaround should basically be considered.

The first approach to reduce the computation cost is to compute eigenvectors (or singular vectors for rectangular matrices) approximately \cite{fowlkes04, oh15}. They drastically reduce the computation cost. One drawback of this approximate eigendecomposition approach is that we have to decide how many eigenvectors are used prior to the decomposition. In contrast to the DFT, frequency spacing of the graph Fourier transform, i.e., eigenvalue distribution of the graph Laplacian, is nonuniform and heavily depends on the graph used.
% Therefore, the value itself is more important than the number of eigenvalues.

The second approach is polynomial approximation of the spectral response $\widetilde{h}(\lambda)$ \cite{saad84, kokiopoulou04, zhou07, cai13, onuki17}. Generally, if the filter response in the graph spectral domain is a $K$th order polynomial function $\widetilde{h}(\lambda) = \sum_{k=0}^{K-1} a_k \lambda^k$, it can be represented as $K$ matrix-vector multiplications \cite{shuman13} since
\begin{equation}
\label{ }
\mathbf{U}\widetilde{h}(\mathbf{\Lambda})\mathbf{U}^T = \mathbf{U}\left(\sum_{k=0}^{K-1} a_k \mathbf{\Lambda}^k \right)\mathbf{U}^T = \sum_{k=0}^{K-1} a_k \mathbf{L}^k,
%\begin{split}
%\mathbf{H} & = \mathbf{U}\widetilde{h}(\mathbf{\Lambda})\mathbf{U}^T\\
%& = \mathbf{U}\left(\sum_{k=0}^{K-1} a_k \mathbf{\Lambda}^k \right)\mathbf{U}^T\\
%& = \sum_{k=0}^{K-1} a_k \mathbf{L}^k,
%\end{split}
\end{equation}
where we utilize the fact $\mathbf{L}^k = \mathbf{U}\mathbf{\Lambda}^k\mathbf{U}^T$. The $K$th order polynomial function on the graph can also be represented as the $K$-hop neighborhood transform in the vertex domain \cite{shuman13}. Especially for the graph spectral filter, we do not need the specific eigenvalues and eigenvectors but the filtered signal (pixel values). Therefore, this approach generally works well for image filtering using graph spectral analysis.

Among the polynomial approximation methods, Chebyshev polynomial approximation \cite{mason02, phillips03, hammond11, shuman11, onuki17} is widely used for graph signal processing from some reasons. First, it can calculate with a recurrence relation; Memory requirement is small. Second, it produces low errors for the passband region. Third, it is very close to minimax polynomial and error bound can be calculated. Its approximation error for $\widetilde{h}(\lambda) = e^{-\lambda}$ is shown in Fig. \ref{fig:approxerror}. As compared with the Taylor series, the error by the Chebyshev approximation is bounded for all range of $\lambda$.

%Let $\widetilde{h}(\lambda)$ be a (non-polynomial) spectral response of the graph filter defined on the interval $\lambda \in [0, \lambda_{\max}]$ and $\widetilde{h}(\mathbf{L}) := \mathbf{U} \text{diag}(\widetilde{h}(\lambda_1), \widetilde{h}(\lambda_2), \ldots, \widetilde{h}(\lambda_{\max})) \mathbf{U}^T$. The approximated response using the $K$th order Chebyshev polynomial approximation is represented as follows \cite{mason02, phillips03, hammond11, saad84, zhou07, lin16}:
%\begin{equation}
%\label{ }
%\widehat{h}(\mathbf{L}) = \frac{1}{2}c_0 \mathbf{I} + \sum_{k=1}^{K-1} c_k \psi_k(\mathbf{L}),
%\end{equation}
%where $c_k\ (k = 0, \ldots, K-1)$ is the Chebyshev coefficient and $\psi_k(\mathbf{L})$ is the Chebyshev polynomial. $\psi_k(\mathbf{L})$ has the following recurrence relation:
%\begin{equation}
%\label{ }
%\psi_k(\mathbf{L}) = \frac{4}{\lambda_{\max}}(\mathbf{L} - \mathbf{I})\psi_{k-1}(\mathbf{L})-\psi_{k-2}(\mathbf{L})
%\end{equation}
%where $\psi_0(\mathbf{L}) = \mathbf{I}$ and $\psi_1(\mathbf{L}) = 2(\mathbf{L} - \mathbf{I})/\lambda_{\max}$. Furthermore, the Chebyshev coefficient is calculated as
%\begin{equation}
%\label{ }
%\begin{split}
%c_k = \frac{1}{K_s} \sum_{m=1}^{K_s}& \cos\left(\frac{\pi k \left(m - \frac{1}{2}\right)}{K_a}\right)\\
%&\times \widetilde{h}\left(\frac{\lambda_{\max}}{2} \left(\cos\left(\frac{\pi \left(m-\frac{1}{2}\right)}{K_s}\right) + 1\right)\right)
%\end{split}
%\end{equation}
%where $K_s$ is the number of sampling points used to compute the Chebyshev coefficients and is usually set to $K_s = K + 1$.
%\begin{equation}
%\label{ }
%c_k = \frac{2}{\pi} \int_{0}^{\pi} \cos(k \theta) h\left(\frac{\cos\theta + 1}{2}\lambda_{\max}\right) d\theta.
%\end{equation}
The computational complexity of the $K$th order Chebyshev approximation is $O(K(|E| + N))$, where $|E|$ is the number of edges, which is generally much lower than $O(N^3)$ of the full eigendecomposition (via the QR algorithm) \cite{golub96, hammond11, sakiyama16, onuki17}.









































